Efficient Conditional Pre-training for Transfer Learning

Almost all the state-of-the-art neural networks for computer vision tasks are trained by (1) pre-training on a large-scale dataset and (2) finetuning on the target dataset. This strategy helps reduce dependence on the target dataset and improves convergence rate and generalization on the target task. Although pre-training on large-scale datasets is very useful, its foremost disadvantage is high training cost. To address this, we propose efficient filtering methods to select relevant subsets from the pre-training dataset. Additionally, we discover that lowering image resolutions in the pre-training step offers a great trade-off between cost and performance. We validate our techniques by pre-training on ImageNet in both the unsupervised and supervised settings and finetuning on a diverse collection of target datasets and tasks. Our proposed methods drastically reduce pre-training cost and provide strong performance boosts. Finally, we improve standard ImageNet pre-training by 1-3% by tuning available models on our subsets and pre-training on a dataset filtered from a larger scale dataset.

==> Sections/Discussion.tex <==
\section{Discussion}
\subsubsection{Effect of resolution}
\subsubsection{Comparison of filtering methods}
\subsubsection{Supervised vs Unsupervised}
\subsubsection{Future Directions}

==> Sections/Introduction_2.tex <==
Recent success of modern computer vision methods relies heavily on large-scale labelled datasets, which are often costly to collect~\cite{mahajan2018exploring,he2019momentum,chen2020improved}. Alternatives to large-scale labelled data include pre-training a network on the publicly available ImageNet dataset with labels~\cite{deng2009imagenet} and performing transfer learning on target tasks~\cite{huh2016makes,xie2015transfer,shin2016deep,hendrycks2019using,kornblith2019better}. On the other hand, unsupervised learning has received tremendous attention recently with the availability of extremely large-scale data with no labels, as such data is costly to obtain ~\cite{mahajan2018exploring,he2019momentum,he2020momentum,grill2020bootstrap,caron2020unsupervised,chen2020simple, chen2020improved}. 
%It has been shown that recent unsupervised learning methods, e.g. contrastive learning, can perform on par with their supervised learning counterparts~\cite{he2019momentum,he2020momentum,grill2020bootstrap,caron2020unsupervised,chen2020simple, chen2020improved} and even better in certain settings~\cite{he2019momentum,he2020momentum,chen2020improved}.

The explosion of data quantity and improvement of unsupervised learning with contrastive learning portends that the standard approach in future tasks will be to (1) learn weights a on a very large-scale dataset with unsupervised learning and (2) fine-tune them on a small-scale target dataset. A major problem with this approach is the large amount of computational resources required to train a network on a very large scale dataset~\cite{mahajan2018exploring}. For example, a recent contrastive learning method, MoCo-v2~\cite{he2020momentum,he2019momentum}, uses 8 GPUs to train on ImageNet for 53 hours, which can cost thousands of dollars. Extrapolating, this forebodes pre-training costs on the order of millions of dollars on larger-scale datasets. Those without access to such computation power will require selecting relevant subsets of those datasets specific to their task. 
%However, other studies that perform conditional filtering, such as ~\cite{Yan_2020_CVPR,cui2018large,ngiam2018domain,ge2017borrowing}, do not consider efficiency.

Cognizant of these pressing issues, we propose novel methods to efficiently filter a user defined number of pre-training images conditioned on a target dataset. 
%as well as a novel sequential pre-training method for our methods to work efficiently in practical settings with several target tasks
%\burak{This is confusing. Sequential pre-training comes out of nowhere. we should keep this part simple and highlight the results. I changed this paragraph, have a look.}. 
We also find that the use of low resolution images during pre-training provides a great cost to performance trade-off. Our approach consistently outperforms other methods
%~\burak{What methods? Filtering?} 
by $2\text{-}9\%$ and are both flexible, translating to both supervised and unsupervised settings, and adaptable, translating to a wide range of target tasks including image recognition, object detection and semantic segmentation. Our methods perform especially well in the more relevant unsupervised setting where pre-training on a $12\%$ subset of data can achieve within $1\text{-}4\%$ of full pre-training when considering target task performance. Next, we use our methods to improve standard ImageNet (1.28M images) pre-training. In this direction, we construct a large scale dataset (6.7M images) from multiple datasets and filter 1.28M images conditioned on a target task. Our results show that we improve standard ImageNet pre-training by $1\text{-}3\%$ on downstream tasks. Thus, when needing to pre-train from scratch on large scale data for a specific application, our methods can replace the standard ImageNet pre-training %and current filtering methods 
with conditional pre-training.
% Our methods are promising and well suited to take advantage of the availability of larger scale data and increasing popularity of unsupervised learning to enhance  
